MultiPhys: Multi-Person Physics-aware 3D Motion Estimation

We introduce MultiPhys, a method designed for recovering multi-person motion from monocular videos. Our focus lies in capturing coherent spatial placement between pairs of individuals across varying degrees of engagement. MultiPhys, being physically aware, exhibits robustness to jittering and occlusions, and effectively eliminates penetration issues between the two individuals. We devise a pipeline in which the motion estimated by a kinematic-based method is fed into a physics simulator in an autoregressive manner. We introduce distinct components that enable our model to harness the simulator's properties without compromising the accuracy of the kinematic estimates. This results in final motion estimates that are both kinematically coherent and physically compliant. Extensive evaluations on three challenging datasets characterized by substantial inter-person interaction show that our method significantly reduces errors associated with penetration and foot skating, while performing competitively with the state-of-the-art on motion accuracy and smoothness. Results and code can be found on our project page (http://www.iri.upc.edu/people/nugrinovic/multiphys/).

==> figures/ablation_loopN.tex <==
% \begin{figure}[h!]
\begin{figure*}[h!]
\centering
\includegraphics[width=1\linewidth]{imgs/ablation-loopN_2.pdf} \\[-0.2cm]
\caption{
\textbf{Effect of the \loopN component} \nicolas{draft, maybe not include this figure in the paper} This is an extreme case that showcases... 
\vspace*{-0.3cm}
}
\label{fig:loopN}
\end{figure*}

==> figures/loopN.tex <==
% \begin{figure}[h!]
\begin{figure}[]
\centering
\includegraphics[width=1\linewidth]{imgs/loopN.pdf} \\[-0.2cm]
\caption{
\textbf{\loopN component.} Text here \nuk{Raw draft, quality should be improved}. 
\vspace*{-0.3cm}
}
\label{fig:loopN}
\end{figure}

==> tables/ablation_hi4d.tex <==
\begin{table*}[]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{l cccc Hcc}
\toprule
Method & Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA   \\
\midrule
% SLAHMR~\cite{ye2023slahmr}       & 367.3         & 12.2         & 4.9          & \textbf{6.9} & \textbf{80.9} & 121.6    & \textbf{69.1}  \\
% Baseline     & \textbf{39.8} & 3.8          & \textbf{1.3} & 12.7         & 115.3         & 148.8          & 92.9          \\
Ours (Loop1) & {\ul 49.2}    & \textbf{2.4} & {\ul 2.6}    & {\ul9.2}     & 88.4          & 121.1          & 73.1          \\
Ours (Loop2) & 51.1          & \textbf{2.4} & 3.5          & 9.6          & {\ul84.8} & {\ul 118.1}    & {\ul 71.2} \\
Ours (Loop3) & 51.0          & \textbf{2.4} & 4.0          & 9.5       & 84.9    & \textbf{118.0} & 71.4    \\
Ours (Loop4) & 50.7          & {\ul 2.5}    & 4.4          & {\ul 9.2}     & 85.0          & 118.2          & 71.7          \\
Ours (Loop5) & 52.2          & {\ul 2.5}    & 4.7          & 9.8          & 85.2          & 118.2          & 71.6    \\
\bottomrule
\end{tabular}
} \\[-0.2cm]
\caption{\textbf{Ablation of the proposed system on Hi4D~\cite{yin2023hi4d}.} We report Pen. in m, Gnd Pen. in mm, Skating in mm W-MPJPE and PA-MPJPE in mm, Acc Error in mm/s\textsuperscript{2}. We choose $\nloop=2$ for the rest of the experiments as it provides a good balance between physics and pose metrics.
}
\label{tab:ablation}
\end{table*}




==> tables/sota_bck.tex <==
\begin{table*}[]
\centering
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{l cccc Hcc}
\toprule


\multicolumn{8}{c}{CHI3D} \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA   \\
\midrule
SLAHMR~\cite{ye2023slahmr}          & 139.3         & 4.4          & \textbf{1.0} & \textbf{6.5} & {\ul 100.9}    & {\ul 177.1}    & {\ul 83.5}     \\
EmbPose-MP~\cite{Luo2022EmbodiedSH}        & {\ul 40.2}    & \textbf{2.6} & 2.8          & 7.7          & 126.7          & 214.7          & 96.5           \\
Ours            & \textbf{18.7} & {\ul 3.2}    & {\ul 2.7}    & {\ul 7.4}    & \textbf{98.1}  & \textbf{174.7} & \textbf{80.4}  \\
\midrule
\multicolumn{8}{c}{Hi4D}    \\ 
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR~\cite{ye2023slahmr}          & 367.3         & 12.2         & 4.9          & \textbf{6.9} & \textbf{80.9}  & {\ul 121.6}    & \textbf{69.1}  \\
EmbPose-MP~\cite{Luo2022EmbodiedSH} & \textbf{39.8} & {\ul 3.8}    & \textbf{1.3} & 12.7         & 115.3          & 148.8          & 92.9           \\
Ours            & {\ul 51.1}    & \textbf{2.4} & {\ul 3.5}    & {\ul 9.6}    & {\ul 84.8}     & \textbf{118.1} & {\ul 71.2}     \\
\midrule
\multicolumn{8}{c}{ExPI}  \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR~\cite{ye2023slahmr}          & 567.3         & 18.6         & 5.4          & \textbf{8.2} & \textbf{187.3} & {\ul 263.3}    & \textbf{159.1} \\
EmbPose-MP~\cite{Luo2022EmbodiedSH}        & {\ul 92.1}    & {\ul 0.9}    & \textbf{1.9} & 27.7         & 288.6          & 386.4          & 207.6          \\
Ours            & \textbf{73.0} & \textbf{0.6} & {\ul 2.3}    & {\ul 17.1}   & {\ul 196.3}    & \textbf{250.9} & {\ul 164.3}   \\
\bottomrule
\end{tabular}
} \\[-0.2cm]
\caption{\textbf{Comparison with the state of the art.} We report various metrics on CHI3D~\cite{Fieraru_2020_CVPR}, Hi4D~\cite{yin2023hi4d}, and ExPI~\cite{guo2021multi} datasets. Pose metrics are W-MPJPE and PA-MPJPE (joint) in mm. See ~\cref{subsec:experiments:comparison}.
% \vspace*{-0.4cm}
}
\label{tab:sota}
\end{table*}
% \vspace*{-0.3cm}


==> tables/sota_kin.tex <==
\begin{table}[]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l HHHc Hcc}
\toprule
\multicolumn{8}{c}{CHI3D} \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA   \\
\midrule
SLAHMR          & 139.3         & 4.4          & \textbf{1.0} & \textbf{6.5} & {\ul 100.9}    & {\ul 177.1}    & {\ul 83.5}     \\
Baseline        & {\ul 40.2}    & \textbf{2.6} & 2.8          & 7.7          & 126.7          & 214.7          & 96.5           \\
Ours            & \textbf{18.7} & {\ul 3.2}    & {\ul 2.7}    & {\ul 7.4}    & \textbf{98.1}  & \textbf{174.7} & \textbf{80.4}  \\
\midrule
\multicolumn{8}{c}{Hi4D}    \\ 
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 367.3         & 12.2         & 4.9          & \textbf{6.9} & \textbf{80.9}  & {\ul 121.6}    & \textbf{69.1}  \\
Baseline (EmbP) & \textbf{39.8} & {\ul 3.8}    & \textbf{1.3} & 12.7         & 115.3          & 148.8          & 92.9           \\
Ours            & {\ul 51.1}    & \textbf{2.4} & {\ul 3.5}    & {\ul 9.6}    & {\ul 84.8}     & \textbf{118.1} & {\ul 71.2}     \\
\midrule
\multicolumn{8}{c}{ExPI}  \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 567.3         & 18.6         & 5.4          & \textbf{8.2} & \textbf{187.3} & {\ul 263.3}    & \textbf{159.1} \\
Baseline        & {\ul 92.1}    & {\ul 0.9}    & \textbf{1.9} & 27.7         & 288.6          & 386.4          & 207.6          \\
Ours            & \textbf{73.0} & \textbf{0.6} & {\ul 2.3}    & {\ul 17.1}   & {\ul 196.3}    & \textbf{250.9} & {\ul 164.3}   \\
\bottomrule
\end{tabular}
} \\[-0.2cm]
\caption{\textbf{Comparison with the state of the art.} We report various metrics on CHI3D~\cite{Fieraru_2020_CVPR}, Hi4D~\cite{yin2023hi4d}, and ExPI~\cite{guo2021multi} datasets. Pose metrics are W-MPJPE and PA-MPJPE (joint) in mm. See Section~\ref{sec:experiments:results}.
\vspace*{-0.4cm}
}
\label{tab:sota_phys}
\end{table}
% \vspace*{-0.3cm}

==> tables/sota_phys.tex <==
\begin{table}[h!]
\centering
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{l ccc HHHH}
\toprule
\multicolumn{8}{c}{CHI3D} \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA   \\
\midrule
SLAHMR          & 139.3         & 4.4          & \textbf{1.0} & \textbf{6.5} & {\ul 100.9}    & {\ul 177.1}    & {\ul 83.5}     \\
Baseline        & {\ul 40.2}    & \textbf{2.6} & 2.8          & 7.7          & 126.7          & 214.7          & 96.5           \\
Ours            & \textbf{18.7} & {\ul 3.2}    & {\ul 2.7}    & {\ul 7.4}    & \textbf{98.1}  & \textbf{174.7} & \textbf{80.4}  \\
\midrule
\multicolumn{8}{c}{Hi4D}    \\ 
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 367.3         & 12.2         & 4.9          & \textbf{6.9} & \textbf{80.9}  & {\ul 121.6}    & \textbf{69.1}  \\
Baseline (EmbP) & \textbf{39.8} & {\ul 3.8}    & \textbf{1.3} & 12.7         & 115.3          & 148.8          & 92.9           \\
Ours            & {\ul 51.1}    & \textbf{2.4} & {\ul 3.5}    & {\ul 9.6}    & {\ul 84.8}     & \textbf{118.1} & {\ul 71.2}     \\
\midrule
\multicolumn{8}{c}{ExPI}  \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 567.3         & 18.6         & 5.4          & \textbf{8.2} & \textbf{187.3} & {\ul 263.3}    & \textbf{159.1} \\
Baseline        & {\ul 92.1}    & {\ul 0.9}    & \textbf{1.9} & 27.7         & 288.6          & 386.4          & 207.6          \\
Ours            & \textbf{73.0} & \textbf{0.6} & {\ul 2.3}    & {\ul 17.1}   & {\ul 196.3}    & \textbf{250.9} & {\ul 164.3}   \\
\bottomrule
\end{tabular}
} \\[-0.2cm]
\caption{\textbf{Comparison with the state of the art.} We report various metrics on CHI3D~\cite{Fieraru_2020_CVPR}, Hi4D~\cite{yin2023hi4d}, and ExPI~\cite{guo2021multi} datasets. Pose metrics are W-MPJPE and PA-MPJPE (joint) in mm. See Section~\ref{sec:experiments:results}.
\vspace*{-0.4cm}
}
\label{tab:sota_kin}
\end{table}
\vspace*{-0.3cm}


\begin{table}[h!]
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l HHHc Hcc}
\toprule
\multicolumn{8}{c}{CHI3D} \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA   \\
\midrule
SLAHMR          & 139.3         & 4.4          & \textbf{1.0} & \textbf{6.5} & {\ul 100.9}    & {\ul 177.1}    & {\ul 83.5}     \\
Baseline        & {\ul 40.2}    & \textbf{2.6} & 2.8          & 7.7          & 126.7          & 214.7          & 96.5           \\
Ours            & \textbf{18.7} & {\ul 3.2}    & {\ul 2.7}    & {\ul 7.4}    & \textbf{98.1}  & \textbf{174.7} & \textbf{80.4}  \\
\midrule
\multicolumn{8}{c}{Hi4D}    \\ 
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 367.3         & 12.2         & 4.9          & \textbf{6.9} & \textbf{80.9}  & {\ul 121.6}    & \textbf{69.1}  \\
Baseline (EmbP) & \textbf{39.8} & {\ul 3.8}    & \textbf{1.3} & 12.7         & 115.3          & 148.8          & 92.9           \\
Ours            & {\ul 51.1}    & \textbf{2.4} & {\ul 3.5}    & {\ul 9.6}    & {\ul 84.8}     & \textbf{118.1} & {\ul 71.2}     \\
\midrule
\multicolumn{8}{c}{ExPI}  \\
\midrule
Method &  Pen.\doA  & Gnd Pen.\doA  & Skating\doA  & Acc. Error\doA &  WA-MPJPE\doA  & W-MPJPE\doA  & PA-MPJPE (joint)\doA    \\
\midrule
SLAHMR          & 567.3         & 18.6         & 5.4          & \textbf{8.2} & \textbf{187.3} & {\ul 263.3}    & \textbf{159.1} \\
Baseline        & {\ul 92.1}    & {\ul 0.9}    & \textbf{1.9} & 27.7         & 288.6          & 386.4          & 207.6          \\
Ours            & \textbf{73.0} & \textbf{0.6} & {\ul 2.3}    & {\ul 17.1}   & {\ul 196.3}    & \textbf{250.9} & {\ul 164.3}   \\
\bottomrule
\end{tabular}
} \\[-0.2cm]
\caption{\textbf{Comparison with the state of the art.} We report various metrics on CHI3D~\cite{Fieraru_2020_CVPR}, Hi4D~\cite{yin2023hi4d}, and ExPI~\cite{guo2021multi} datasets. Pose metrics are W-MPJPE and PA-MPJPE (joint) in mm. See Section~\ref{sec:experiments:results}.
\vspace*{-0.4cm}
}
\label{tab:sota_phys}
\end{table}
% \vspace*{-0.3cm}
